Hardware-Centric AutoML for Mixed-Precision Quantization

Model quantization is a widely used technique to compress and accelerate deep neural network (DNN) inference. Emergent DNN hardware accelerators begin to support mixed precision (1-8 bits) to further improve the computation efficiency, which raises a great challenge to find the optimal bitwidth for each layer: it requires domain experts to explore the vast design space trading off among accuracy, latency, energy, and model size, which is both time-consuming and sub-optimal. Conventional quantization algorithm ignores the different hardware architectures and quantizes all the layers in a uniform way. In this paper, we introduce the Hardware-Aware Automated Quantization (HAQ) framework which leverages the reinforcement learning to automatically determine the quantization policy, and we take the hardware accelerator's feedback in the design loop. Rather than relying on proxy signals such as FLOPs and model size, we employ a hardware simulator to generate direct feedback signals (latency and energy) to the RL agent. Compared with conventional methods, our framework is fully automated and can specialize the quantization policy for different neural network architectures and hardware architectures. Our framework effectively reduced the latency by 1.4-1.95x and the energy consumption by 1.9x with negligible loss of accuracy compared with the fixed bitwidth (8 bits) quantization. Our framework reveals that the optimal policies on different hardware architectures (i.e., edge and cloud architectures) under different resource constraints (i.e., latency, energy, and model size) are drastically different. We interpreted the implication of different quantization policies, which offer insights for both neural network architecture design and hardware architecture design.

==> figText/detail_bismo_mobilenetv2.tex <==
\begin{table}[!t]
    \renewcommand*{\arraystretch}{1.1}
    \setlength{\tabcolsep}{2pt}
    \small\centering
    \begin{tabular}{lcccccccc}
        \toprule
        ID & Type & Channels & Weights & Activation & Latency & GOps/s & Ops/Byte &  \\
        \midrule
        1 & D & 3 & 8 bits & 8 bits & 2.15 ms & 82 & 76 \\
        2 & P & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        3 & D & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        4 & D & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        5 & P & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        6 & D & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        7 & D & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        8 & P & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        9 & D & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        10 & D & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        11 & P & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        12 & D & 3 & 4 bits & 4 bits & 2.15 ms & 82 & 76 \\
        \bottomrule
    \end{tabular}
    \caption{Comparisons between our agent's transfer results (from MobileNet-V1 to MobileNet-V2), its direct search results on MobileNet-V2, and the fixed-bitwidth baseline (PACT). Our RL agent is able to generalize well to different network architectures: our quantization policy transferred from V1 to V2 performs better than the fixed-bitwidth baseline and is only slighly worse than the quantization policy directly searched fro V2.}
    \label{tbl:bismo_transfer}
\end{table}

==> figText/detail_policy.tex <==
% \begin{table}[!t]
%     \renewcommand*{\arraystretch}{1.2}
%     \setlength{\tabcolsep}{5pt}
%     \small\centering
%     \begin{tabular}{lcccc}
%         \toprule
%         & Bitwidth & Acc.-1 & Acc.-5 & Latency \\
%         \midrule
%         PACT & 4 bits & 61.39 & 83.72 & 52.15 ms \\
%         Ours (search for V2) & \emph{flexible} & 66.99 & 87.33 & 52.12 ms \\
%         Ours (transfer from V1) & \emph{flexible} & 65.80 & 86.60 & 52.06 ms \\
%         \midrule
%         PACT & 5 bits & 68.84 & 88.58 & 66.94 ms \\
%         Ours (search for V2) & \emph{flexible} & 70.90 & 89.91 & 66.92 ms \\
%         Ours (transfer from V1) & \emph{flexible} & 69.90 & 89.24 & 66.93 ms \\
%         \bottomrule
%     \end{tabular}
%     \caption{\ijcv{Comparisons between our agent's transfer results (from MobileNet-V1 to MobileNet-V2), its direct search results on MobileNet-V2, and the fixed-bitwidth baseline (PACT). Our RL agent is able to generalize well to different network architectures: our quantization policy transferred from V1 to V2 performs better than the fixed-bitwidth baseline and is only slighly worse than the quantization policy directly searched fro V2.}}
%     \label{tbl:bismo_transfer}
% \end{table}

\begin{table*}[!t]
    \renewcommand*{\arraystretch}{1.}
    \setlength{\tabcolsep}{0.5pt}
    \small\centering
    \begin{tabular}{lccccccccccccccccccccccccccccccccccccccccccccccccccccccc} 
        \toprule
        id: & ~1 & ~2 & ~3 & ~4 & ~5 & ~6 & ~7 & ~8 & ~9 & 10 & 11 & 12 & 13 & 14 & 15 & 16 & 17 & 18 & 19 & 20 & 21 & 22 & 23 & 24 & 25 & 26 & 27 & 28 & 29 & 30 & 31 & 32 & 33 & 34 & 35 & 36 & 37 & 38 & 39 & 40 & 41 & 42 & 43 & 44 & 45 & 46 & 47 & 48 & 49 & 50 & 51 & 52 \\
        \midrule
        w: & 8 & 3 & 2 & 5 & 6 & 5 & 5 & 5 & 6 & 5 & 5 & 5 & 5 & 6 & 5 & 5 & 5 & 5 & 5 & 6 & 5 & 6 & 5 & 5 & 6 & 5 & 4 & 6 & 5 & 4 & 5 & 5 & 4 & 5 & 6 & 4 & 5 & 6 & 5 & 4 & 6 & 5 & 4 & 6 & 5 & 3 & 6 & 5 & 3 & 6 & 6 & 8 \\
        \midrule
        a: & 8 & 6 & 7 & 4 & 6 & 6 & 3 & 6 & 5 & 3 & 6 & 5 & 3 & 6 & 5 & 3 & 6 & 5 & 4 & 5 & 6 & 4 & 6 & 7 & 3 & 6 & 5 & 4 & 5 & 5 & 4 & 6 & 6 & 4 & 6 & 5 & 4 & 6 & 6 & 5 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 8 \\
        \midrule
        w: & 8 & 3 & 2 & 5 & 6 & 5 & 5 & 5 & 6 & 5 & 5 & 5 & 5 & 6 & 5 & 5 & 5 & 5 & 5 & 6 & 5 & 6 & 5 & 5 & 6 & 5 & 4 & 6 & 5 & 4 & 5 & 5 & 4 & 5 & 6 & 4 & 5 & 6 & 5 & 4 & 6 & 5 & 4 & 6 & 5 & 3 & 6 & 5 & 3 & 6 & 6 & 8 \\
        \midrule
        a: & 8 & 6 & 7 & 4 & 6 & 6 & 3 & 6 & 5 & 3 & 6 & 5 & 3 & 6 & 5 & 3 & 6 & 5 & 4 & 5 & 6 & 4 & 6 & 7 & 3 & 6 & 5 & 4 & 5 & 5 & 4 & 6 & 6 & 4 & 6 & 5 & 4 & 6 & 6 & 5 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 8 \\
        \midrule
        w: & 8 & 3 & 2 & 5 & 6 & 5 & 5 & 5 & 6 & 5 & 5 & 5 & 5 & 6 & 5 & 5 & 5 & 5 & 5 & 6 & 5 & 6 & 5 & 5 & 6 & 5 & 4 & 6 & 5 & 4 & 5 & 5 & 4 & 5 & 6 & 4 & 5 & 6 & 5 & 4 & 6 & 5 & 4 & 6 & 5 & 3 & 6 & 5 & 3 & 6 & 6 & 8 \\
        \midrule
        a: & 8 & 6 & 7 & 4 & 6 & 6 & 3 & 6 & 5 & 3 & 6 & 5 & 3 & 6 & 5 & 3 & 6 & 5 & 4 & 5 & 6 & 4 & 6 & 7 & 3 & 6 & 5 & 4 & 5 & 5 & 4 & 6 & 6 & 4 & 6 & 5 & 4 & 6 & 6 & 5 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 6 & 8 \\
        \bottomrule
     
    \end{tabular}
    \caption{Latency-constrained quantization on BISMO (edge accelerator and cloud accelerator) on ImageNet. Our framework can reduce the latency by \textbf{1.4$\times$} to \textbf{1.95$\times$} with negligible loss of accuracy compared with the fixed bitwidth (8 bits) quantization.}
    \label{tbl:bismo_latency}
\end{table*}

==> figText/exploration_curves.tex <==
\begin{figure*}[htb]
    \centering
    \includegraphics[width=1.0\linewidth]{figures/search_curves.pdf}
    \caption{Exploration curves of resource-constrained quantization (for MobileNet-V1 on 100-category subset of ImageNet).}
    \label{fig:exploration_curves}
\end{figure*}

==> figText/figures/agent.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{figures/agent.pdf}
    \caption{The network configuration of our actor critic agent.}
    \label{fig:agent}
\end{figure}

==> figText/full_detail_policy.tex <==
\begin{table}[!t]
    \renewcommand*{\arraystretch}{1.2}
    \setlength{\tabcolsep}{5pt}
    \small\centering
    \begin{tabular}{lcccc}
        \toprule
        & Bitwidth & Acc.-1 & Acc.-5 & Latency \\
        \midrule
        PACT & 4 bits & 61.39 & 83.72 & 52.15 ms \\
        Ours (search for V2) & \emph{flexible} & 66.99 & 87.33 & 52.12 ms \\
        Ours (transfer from V1) & \emph{flexible} & 65.80 & 86.60 & 52.06 ms \\
        \midrule
        PACT & 5 bits & 68.84 & 88.58 & 66.94 ms \\
        Ours (search for V2) & \emph{flexible} & 70.90 & 89.91 & 66.92 ms \\
        Ours (transfer from V1) & \emph{flexible} & 69.90 & 89.24 & 66.93 ms \\
        \bottomrule
    \end{tabular}
    \caption{Comparisons between our agent's transfer results (from MobileNet-V1 to MobileNet-V2), its direct search results on MobileNet-V2, and the fixed-bitwidth baseline (PACT). Our RL agent is able to generalize well to different network architectures: our quantization policy transferred from V1 to V2 performs better than the fixed-bitwidth baseline and is only slighly worse than the quantization policy directly searched fro V2.}
    \label{tbl:bismo_transfer}
\end{table}


